M Dwarf Activity in the Pan-STARRS 1 Medium-Deep Survey: First Catalog and Rotation Periods

We report on an ongoing project to investigate activity in the M dwarf stellar population observed by the Pan-STARRS 1 Medium Deep Survey (PS1-MDS). Using a custom-built pipeline, we refine an initial sample of $\approx$ 4 million sources in PS1-MDS to a sample of 184,148 candidate cool stars using color cuts. Motivated by the well-known relationship between rotation and stellar activity, we use a multi-band periodogram analysis and visual vetting to identify 271 sources that are likely rotating M dwarfs. We derive a new set of polynomials relating M dwarf PS1 colors to fundamental stellar parameters and use them to estimate the masses, distances, effective temperatures, and bolometric luminosities of our sample. We present a catalog containing these values, our measured rotation periods, and cross-matches to other surveys. Our final sample spans periods of $\lesssim$1-130 days in stars with estimated effective temperatures of $\approx$ 2700-4000 K. Twenty-two of our sources have X-ray cross-matches, and they are found to be relatively X-ray bright as would be expected from selection effects. Our data set provides evidence that Kepler-based searches have not been sensitive to very slowly-rotating stars ($P_{\rm rot} \gtrsim 70$ d), implying that the observed emergence of very slow rotators in studies of low-mass stars may be a systematic effect. We also see a lack of low-amplitude ($<$2%) variability in objects with intermediate (10-40 d) rotation periods, which, considered in conjunction with other observational results, may be a signpost of a loss of magnetic complexity associated with a phase of rapid spin-down in intermediate-age M dwarfs. This work represents just a first step in exploring stellar variability in data from the PS1-MDS and, in the farther future, LSST.

==> rotators-full.tex <==
% TableBuilder table
\begin{deluxetable}{lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lr@{}l@{\,}lcr@{}l@{\,}lr@{}lr@{}lc}
%custom preamble
\tabletypesize{\tiny}
%hardcoded preamble
\tablecolumns{37}
\tablewidth{0em}
\tablecaption{Candidate Rotating M~Dwarfs\label{t.rotators}}
\tablehead{
\colhead{Name} & \multicolumn{3}{c}{$z_\text{P1}$} & \multicolumn{3}{c}{$(g-r)_\text{P1}$} & \multicolumn{3}{c}{$(r-i)_\text{P1}$} & \multicolumn{3}{c}{$(i-z)_\text{P1}$} & \multicolumn{3}{c}{$(z-y)_\text{P1}$} & \multicolumn{3}{c}{\teff} & \multicolumn{3}{c}{Mass} & \multicolumn{3}{c}{$d$} & \multicolumn{3}{c}{$\log_{10} L_\text{bol}$} & \colhead{Giant?} & \multicolumn{3}{c}{$P_\text{rot}$} & \multicolumn{2}{c}{Ampl.} & \multicolumn{2}{c}{Pk. Rat.} & \colhead{\paeight} \\
 & \multicolumn{3}{c}{(mag)} & \multicolumn{3}{c}{(mag)} & \multicolumn{3}{c}{(mag)} & \multicolumn{3}{c}{(mag)} & \multicolumn{3}{c}{(mag)} & \multicolumn{3}{c}{(K)} & \multicolumn{3}{c}{(M$_\odot$)} & \multicolumn{3}{c}{(pc)} & \multicolumn{3}{c}{[$L_\odot$]} &  & \multicolumn{3}{c}{(day)} & \multicolumn{2}{c}{(\%)} &  &  &  \\ \\
\multicolumn{1}{c}{(1)} & \multicolumn{3}{c}{(2)} & \multicolumn{3}{c}{(3)} & \multicolumn{3}{c}{(4)} & \multicolumn{3}{c}{(5)} & \multicolumn{3}{c}{(6)} & \multicolumn{3}{c}{(7)} & \multicolumn{3}{c}{(8)} & \multicolumn{3}{c}{(9)} & \multicolumn{3}{c}{(10)} & \multicolumn{1}{c}{(11)} & \multicolumn{3}{c}{(12)} & \multicolumn{2}{c}{(13)} & \multicolumn{2}{c}{(14)} & \multicolumn{1}{c}{(15)}
}
\startdata
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_38_3_0__0.6038602668144477_-0.0842229258309879}{WISEA J021823.69$-$044932.5} & $17$ & $.72$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $3140$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.04$\rule{0pt}{3ex} & $350$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $13$ & $.37$ & $\pm\,0.03$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.71$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_67_4_2__0.6070474355710005_-0.0614468867372131}{WISEA J021907.51$-$033114.2} & $16$ & $.74$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $3060$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $190$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $12$ & $.39$ & $\pm\,0.03$\rule{0pt}{3ex} & $4$ & $.0$ & $2$ & $.30$ & 38 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_76_4_3__0.6139307897161028_-0.0544004859503063}{WISEA J022042.16$-$030701.0} & $16$ & $.38$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $390$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.195$ & $\pm\,0.002$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.37$ & 26 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_56_2_2__0.6144377196236567_-0.0734844536985636}{WISEA J022049.11$-$041237.1} & $19$ & $.41$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,90$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $750$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $25$ & $.57$ & $\pm\,0.10$\rule{0pt}{3ex} & $3$ & $.9$ & $1$ & $.84$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_66_3_0__0.6157135625325550_-0.0626785714391230}{WISEA J022106.66$-$033528.4} & $17$ & $.72$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3260$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $16$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $4$ & $.4$ & $1$ & $.91$ & 41 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_16_3_3__0.6162354277762703_-0.0954191689175081}{WISEA J022113.86$-$052801.8} & $18$ & $.31$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3040$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $360$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.6249$ & $\pm\,0.0006$\rule{0pt}{3ex} & $1$ & $.9$ & $2$ & $.91$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_46_1_3__0.6168143691321055_-0.0789655966518750}{WISEA J022121.80$-$043127.9} & $16$ & $.58$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3370$ & $\pm\,0.0003$\rule{0pt}{3ex} & $1$ & $.2$ & $1$ & $.23$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_45_1_1__0.6234736840804432_-0.0793849087092632}{WISEA J022253.37$-$043254.3} & $16$ & $.87$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.84$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3710$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.09$\rule{0pt}{3ex} & $710$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.203$ & $\pm\,0.004$\rule{0pt}{3ex} & $2$ & $.8$ & $5$ & $.59$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_25_1_2__0.6258051087911054_-0.0946810743719948}{WISEA J022325.43$-$052529.4} & $17$ & $.03$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.08$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3900$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.10$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & P & $36$ & $.2$ & $\pm\,0.3$\rule{0pt}{3ex} & $5$ & $.2$ & $1$ & $.93$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_25_1_2__0.6259300107119000_-0.0933507800555881}{WISEA J022327.16$-$052055.0} & $15$ & $.85$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $200$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.019$ & $\pm\,0.004$\rule{0pt}{3ex} & $1$ & $.9$ & $4$ & $.10$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_24_2_0__0.6283612568084030_-0.0931096846654621}{WISEA J022400.58$-$052005.1} & $16$ & $.36$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3370$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.06$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $60$ & $.9$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.08$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_44_4_0__0.6291731966829420_-0.0743107062807737}{WISEA J022411.77$-$041527.7} & $17$ & $.85$ & $\pm\,0.03$\rule{0pt}{3ex} & \multicolumn{3}{c}{}\rule{0pt}{3ex} & \multicolumn{3}{c}{}\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3170$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $390$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.3451$ & $\pm\,0.0010$\rule{0pt}{3ex} & $4$ & $.1$ & $1$ & $.22$ & 28 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_34_4_0__0.6292787008937766_-0.0841817653639817}{WISEA J022413.20$-$044923.8} & $17$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3400$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $41$ & $.1$ & $\pm\,0.3$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.43$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_24_1_3__0.6299929581579058_-0.0942608340769354}{SDSS J022423.02$-$052402.8} & $19$ & $.38$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $1200$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.4676$ & $\pm\,0.0007$\rule{0pt}{3ex} & $3$ & $.7$ & $1$ & $.60$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_74_3_0__0.6307040653140902_-0.0534851939389707}{WISEA J022432.80$-$030352.1} & $16$ & $.53$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3300$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $17$ & $.75$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.51$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_64_3_1__0.6311620846974171_-0.0635268507188396}{WISEA J022439.10$-$033823.4} & $18$ & $.14$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3400$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.07$\rule{0pt}{3ex} & $700$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.3270$ & $\pm\,0.0005$\rule{0pt}{3ex} & $2$ & $.1$ & $2$ & $.10$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_44_1_1__0.6316307432505854_-0.0811521084734921}{WISEA J022445.54$-$043859.0} & $18$ & $.01$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.2694$ & $\pm\,0.0003$\rule{0pt}{3ex} & $2$ & $.1$ & $2$ & $.17$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_74_3_2__0.6323891473797154_-0.0542753074234242}{WISEA J022455.97$-$030635.2} & $16$ & $.70$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $3880$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $14$ & $.07$ & $\pm\,0.06$\rule{0pt}{3ex} & $2$ & $.2$ & $2$ & $.10$ & 26 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_23_4_2__0.6335314938807073_-0.0887363555793234}{WISEA J022511.68$-$050503.2} & $16$ & $.33$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $210$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.054$ & $\pm\,0.003$\rule{0pt}{3ex} & $1$ & $.5$ & $3$ & $.85$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_43_2_1__0.6349080484900609_-0.0800198431146355}{WISEA J022530.61$-$043505.4} & $16$ & $.71$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3380$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.06$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $122$ &  & $\pm\,6$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.02$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_43_3_3__0.6369535522725346_-0.0748466377003258}{WISEA J022558.75$-$041718.3} & $17$ & $.25$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3490$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.08$\rule{0pt}{3ex} & $620$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $6$ & $.491$ & $\pm\,0.008$\rule{0pt}{3ex} & $1$ & $.5$ & $3$ & $.06$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_63_3_1__0.6385324185967240_-0.0618721104233379}{WISEA J022620.44$-$033242.1} & $19$ & $.29$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.08$\rule{0pt}{3ex} & $2$ & $.16$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.98$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $2950$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $8$ & $.753$ & $\pm\,0.010$\rule{0pt}{3ex} & $7$ & $.4$ & $4$ & $.49$ & 37 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_62_4_0__0.6417737411239252_-0.0632459742234034}{WISEA J022705.01$-$033725.4} & $17$ & $.81$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $440$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $39$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & $2$ & $.5$ & $2$ & $.16$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/1_22_2_2__0.6417763000064395_-0.0944940625936223}{WISEA J022705.06$-$052450.8} & $17$ & $.43$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3470$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $610$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $46$ & $.7$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.12$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_37_2_1__0.9044022795759588_-0.4968439902324283}{WISEA J032716.42$-$282801.3} & $16$ & $.60$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.94$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $2930$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.11$ & $\pm\,0.02$\rule{0pt}{3ex} & $120$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.102$ & $\pm\,0.003$\rule{0pt}{3ex} & $4$ & $.8$ & $1$ & $.11$ & 55 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_57_2_0__0.9048954499637970_-0.4816543848621364}{WISEA J032723.21$-$273548.5} & $15$ & $.44$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.2960$ & $\pm\,0.0004$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.81$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_27_3_3__0.9091019230230492_-0.5002654134453675}{WISEA J032821.05$-$283947.2} & $17$ & $.02$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $410$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.0601$ & $\pm\,0.0010$\rule{0pt}{3ex} & $2$ & $.2$ & $8$ & $.01$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_67_3_0__0.9108836035234490_-0.4720689200291007}{WISEA J032845.55$-$270251.2} & $17$ & $.21$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3590$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $680$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $38$ & $.2$ & $\pm\,0.8$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.59$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_66_1_0__0.9149491818554951_-0.4776663393043848}{WISEA J032941.46$-$272205.7} & $16$ & $.99$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.99$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $2900$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.10$ & $\pm\,0.02$\rule{0pt}{3ex} & $120$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1383$ & $\pm\,0.0003$\rule{0pt}{3ex} & $4$ & $.2$ & $1$ & $.57$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_56_1_3__0.9152993373743620_-0.4836073953015356}{WISEA J032946.29$-$274231.2} & $18$ & $.78$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3760$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.09$\rule{0pt}{3ex} & $2000$ &  & $\pm\,400$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.2883$ & $\pm\,0.0007$\rule{0pt}{3ex} & $7$ & $.1$ & $1$ & $.31$ & 34 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_46_1_1__0.9161025307002654_-0.4893133663126328}{WISEA J032957.31$-$280207.9} & $16$ & $.14$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3130$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1239$ & $\pm\,0.0005$\rule{0pt}{3ex} & $4$ & $.7$ & $1$ & $.81$ & 38 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_86_1_0__0.9180919233320987_-0.4622928629557987}{WISEA J033024.66$-$262914.7} & $17$ & $.81$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.88$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.88$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $3000$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.13$ & $\pm\,0.02$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3380$ & $\pm\,0.0004$\rule{0pt}{3ex} & $2$ & $.9$ & $4$ & $.74$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_15_4_2__0.9190700435010634_-0.5070041591632507}{WISEA J033038.12$-$290257.1} & $15$ & $.85$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3750$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.10$\rule{0pt}{3ex} & $480$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.5859$ & $\pm\,0.0010$\rule{0pt}{3ex} & $4$ & $.4$ & $1$ & $.39$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_64_3_2__0.9307579348276654_-0.4741775253779572}{PSO J053.3285$-$27.1683} & $19$ & $.52$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3280$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $1000$ &  & $\pm\,200$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.79920$ & $\pm\,0.00003$\rule{0pt}{3ex} & $4$ & $.7$ & $2$ & $.11$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_24_1_2__0.9309357004631067_-0.5038857934657469}{WISEA J033321.29$-$285213.8} & $17$ & $.04$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $300$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.280$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.4$ & $3$ & $.81$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_64_1_1__0.9315631672939544_-0.4754737630994806}{WISEA J033329.92$-$271433.4} & $16$ & $.33$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3500$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.432$ & $\pm\,0.002$\rule{0pt}{3ex} & $1$ & $.5$ & $4$ & $.58$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_54_1_1__0.9331906153322873_-0.4830381182643553}{WISEA J033352.33$-$274033.8} & $17$ & $.08$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3410$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.07$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $67$ & $.8$ & $\pm\,1.0$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.03$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_24_3_2__0.9337310814129454_-0.5016423090199664}{WISEA J033359.73$-$284431.1} & $18$ & $.51$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.50$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $660$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $13$ & $.43$ & $\pm\,0.03$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.59$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_13_4_1__0.9359005321793114_-0.5083848924484571}{WISEA J033429.55$-$290741.7} & $16$ & $.55$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3770$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.10$\rule{0pt}{3ex} & $660$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.8648$ & $\pm\,0.0010$\rule{0pt}{3ex} & $3$ & $.6$ & $2$ & $.04$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_33_4_2__0.9375010573917858_-0.4955468634901879}{WISEA J033451.57$-$282333.9} & $16$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3790$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.10$\rule{0pt}{3ex} & $570$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.777$ & $\pm\,0.006$\rule{0pt}{3ex} & $3$ & $.5$ & $3$ & $.48$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_43_3_1__0.9391809984432056_-0.4885852168532086}{WISEA J033514.62$-$275938.4} & $18$ & $.95$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.06$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.81325$ & $\pm\,0.00004$\rule{0pt}{3ex} & $5$ & $.1$ & $2$ & $.11$ & 47 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_23_1_1__0.9404969446883916_-0.5039084866996456}{WISEA J033532.78$-$285218.6} & $18$ & $.47$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.82$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3090$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.04$\rule{0pt}{3ex} & $400$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.176$ & $\pm\,0.004$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.96$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_33_1_2__0.9411895477606619_-0.4965794146538720}{WISEA J033542.28$-$282706.9} & $17$ & $.48$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3430$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.07$\rule{0pt}{3ex} & $590$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.401$ & $\pm\,0.002$\rule{0pt}{3ex} & $2$ & $.9$ & $1$ & $.09$ & 33 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_33_3_2__0.9413295482371551_-0.4926583883884572}{WISEA J033544.22$-$281338.1} & $18$ & $.57$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3270$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $630$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.897$ & $\pm\,0.005$\rule{0pt}{3ex} & $3$ & $.5$ & $4$ & $.62$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_62_1_2__0.9483113719192799_-0.4771631734708889}{WISEA J033720.22$-$272022.1} & $17$ & $.81$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3800$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.10$\rule{0pt}{3ex} & $1200$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.219$ & $\pm\,0.002$\rule{0pt}{3ex} & $2$ & $.9$ & $5$ & $.67$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/2_42_3_3__0.9498425033330887_-0.4855341894275078}{WISEA J033741.28$-$274908.6} & $17$ & $.76$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3080$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $310$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $25$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & $2$ & $.5$ & $2$ & $.03$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_58_1_2__2.2479479978581165_0.7756990608814029}{WISEA J083511.50$+$442639.4} & $15$ & $.80$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $150$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7423$ & $\pm\,0.0002$\rule{0pt}{3ex} & $2$ & $.5$ & $2$ & $.68$ & 32 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_68_1_0__2.2495434184951795_0.7826144572205675}{WISEA J083533.44$+$445025.7} & $16$ & $.05$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $180$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.612$ & $\pm\,0.002$\rule{0pt}{3ex} & $1$ & $.9$ & $3$ & $.58$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_37_4_2__2.2525068022914874_0.7640243311152033}{WISEA J083614.19$+$434631.2} & $16$ & $.05$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.87$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3650$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.09$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.164$ & $\pm\,0.003$\rule{0pt}{3ex} & $2$ & $.3$ & $3$ & $.51$ & 33 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_47_2_3__2.2525940743782940_0.7669544583648039}{WISEA J083615.38$+$435635.8} & $16$ & $.47$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.97$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $2920$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.10$ & $\pm\,0.02$\rule{0pt}{3ex} & $100$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3603$ & $\pm\,0.0007$\rule{0pt}{3ex} & $2$ & $.8$ & $3$ & $.71$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_37_4_3__2.2533519368234955_0.7651230985578098}{WISEA J083625.81$+$435017.9} & $16$ & $.99$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.85$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3750$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.725$ & $\pm\,0.004$\rule{0pt}{3ex} & $1$ & $.7$ & $4$ & $.19$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_67_3_0__2.2546068560554828_0.7840030310762454}{WISEA J083643.08$+$445512.2} & $16$ & $.68$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.82$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.86$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $3050$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $26$ & $.92$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.28$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_47_3_2__2.2559580232296614_0.7725138955502979}{WISEA J083701.66$+$441542.6} & $16$ & $.90$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $2860$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.09$ & $\pm\,0.02$\rule{0pt}{3ex} & $110$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $112$ &  & $\pm\,2$\rule{0pt}{3ex} & $3$ & $.9$ & $1$ & $.01$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_26_2_0__2.2600623884687745_0.7548525159042452}{WISEA J083758.07$+$431459.5} & $17$ & $.82$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $430$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.031$ & $\pm\,0.004$\rule{0pt}{3ex} & $2$ & $.9$ & $3$ & $.30$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_76_4_0__2.2603764100721091_0.7924991498374666}{WISEA J083802.39$+$452424.7} & $16$ & $.43$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3270$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $270$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.567$ & $\pm\,0.002$\rule{0pt}{3ex} & $1$ & $.3$ & $3$ & $.98$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_46_2_3__2.2606024369998527_0.7672460836399085}{WISEA J083805.51$+$435735.9} & $18$ & $.21$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $720$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.34902$ & $\pm\,0.00010$\rule{0pt}{3ex} & $2$ & $.0$ & $2$ & $.20$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_56_2_0__2.2611099912238091_0.7750940212516597}{WISEA J083812.53$+$442434.7} & $16$ & $.45$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.04$\rule{0pt}{3ex} & $3100$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $170$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.0244$ & $\pm\,0.0007$\rule{0pt}{3ex} & $1$ & $.7$ & $5$ & $.67$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_46_1_3__2.2653838883866402_0.7692812846248761}{WISEA J083911.26$+$440435.4} & $17$ & $.25$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.88$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $3600$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $730$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.1879$ & $\pm\,0.0008$\rule{0pt}{3ex} & $1$ & $.8$ & $2$ & $.16$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_16_3_3__2.2657068991847118_0.7521485667576203}{WISEA J083915.69$+$430541.7} & $16$ & $.94$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3270$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $330$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $6$ & $.590$ & $\pm\,0.008$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.58$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_56_3_1__2.2666727661072272_0.7780990466039924}{WISEA J083928.98$+$443454.4} & $16$ & $.75$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3220$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $270$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.071$ & $\pm\,0.006$\rule{0pt}{3ex} & $1$ & $.3$ & $4$ & $.30$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_56_1_2__2.2668465012695069_0.7736547946173030}{WISEA J083931.38$+$441937.6} & $18$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3070$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $410$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $14$ & $.27$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.61$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_45_2_2__2.2718011153365496_0.7688805502812875}{WISEA J084039.50$+$440312.8} & $17$ & $.20$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3710$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.3940$ & $\pm\,0.0006$\rule{0pt}{3ex} & $3$ & $.6$ & $2$ & $.08$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_35_1_3__2.2759158444104717_0.7605117726254617}{WISEA J084136.08$+$433426.5} & $16$ & $.74$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $310$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $29$ & $.2$ & $\pm\,0.6$\rule{0pt}{3ex} & $3$ & $.7$ & $1$ & $.56$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_75_1_3__2.2770976126053597_0.7874356999412926}{WISEA J084152.29$+$450659.8} & $18$ & $.83$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $3790$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.10$\rule{0pt}{3ex} & $1900$ &  & $\pm\,400$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.426$ & $\pm\,0.003$\rule{0pt}{3ex} & $5$ & $.9$ & $3$ & $.98$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_65_1_3__2.2777884405399114_0.7807887998829391}{WISEA J084201.85$+$444409.5} & $16$ & $.99$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.08$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3580$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.08$\rule{0pt}{3ex} & $600$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $12$ & $.46$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.61$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_64_4_1__2.2826357848085461_0.7867123553998742}{WISEA J084308.49$+$450430.9} & $15$ & $.87$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3420$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $13$ & $.52$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.8$ & $2$ & $.13$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_44_3_3__2.2855900942046343_0.7699714665943250}{WISEA J084349.11$+$440658.0} & $15$ & $.72$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.57$ & $\pm\,0.04$\rule{0pt}{3ex} & $0$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3130$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.04$\rule{0pt}{3ex} & $140$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $53$ & $.6$ & $\pm\,0.5$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.24$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_64_1_2__2.2856855927642945_0.7818868906550687}{WISEA J084350.44$+$444755.7} & $17$ & $.73$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.06$\rule{0pt}{3ex} & $510$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.75714$ & $\pm\,0.00010$\rule{0pt}{3ex} & $1$ & $.2$ & $2$ & $.32$ & 9 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_84_1_2__2.2861193420556214_0.7959548094593822}{WISEA J084356.40$+$453617.4} & $17$ & $.44$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.08$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3490$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.08$\rule{0pt}{3ex} & $630$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.199$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.3$ & $3$ & $.39$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_73_4_3__2.2931284347244256_0.7918287763711561}{WISEA J084532.78$+$452206.1} & $17$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3450$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $520$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $50$ & $.2$ & $\pm\,0.4$\rule{0pt}{3ex} & $1$ & $.3$ & $1$ & $.25$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_53_1_3__2.2974475249785868_0.7762385031586152}{WISEA J084632.17$+$442830.6} & $17$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.85$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $3030$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $200$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.9061$ & $\pm\,0.0010$\rule{0pt}{3ex} & $4$ & $.6$ & $14$ & $.09$ & 45 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_63_3_1__2.2974738890344977_0.7872145509977517}{WISEA J084632.52$+$450614.6} & $16$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3430$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $310$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $60$ & $.2$ & $\pm\,0.7$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.06$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_42_4_0__2.2996404609672729_0.7719893786023887}{WISEA J084702.32$+$441354.0} & $17$ & $.96$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.94$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3610$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.09$\rule{0pt}{3ex} & $1000$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $16$ & $.47$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.36$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_62_1_1__2.3053299185821690_0.7805543368883704}{WISEA J084820.54$+$444320.8} & $18$ & $.58$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.87$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.93$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $2980$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.14$ & $\pm\,0.02$\rule{0pt}{3ex} & $310$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $36$ & $.5$ & $\pm\,0.3$\rule{0pt}{3ex} & $3$ & $.4$ & $1$ & $.87$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_32_3_0__2.3068682030670136_0.7660593728571726}{WISEA J084841.70$+$435330.9} & $16$ & $.87$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3640$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.09$\rule{0pt}{3ex} & $590$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.76412$ & $\pm\,0.00007$\rule{0pt}{3ex} & $2$ & $.2$ & $2$ & $.41$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_52_1_1__2.3071674630640087_0.7765789099978745}{WISEA J084845.81$+$442940.9} & $17$ & $.01$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3740$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1053$ & $\pm\,0.0005$\rule{0pt}{3ex} & $3$ & $.4$ & $2$ & $.29$ & 37 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_61_2_3__2.3097460266444827_0.7824378476916597}{WISEA J084921.27$+$444949.2} & $17$ & $.07$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3190$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.04$\rule{0pt}{3ex} & $260$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.3399$ & $\pm\,0.0010$\rule{0pt}{3ex} & $4$ & $.2$ & $17$ & $.31$ & 64 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_41_4_0__2.3131305241790958_0.7698504028304738}{WISEA J085007.80$+$440633.4} & $18$ & $.26$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $440$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $7$ & $.26$ & $\pm\,0.02$\rule{0pt}{3ex} & $2$ & $.9$ & $1$ & $.93$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/3_41_3_1__2.3154689747081081_0.7730319462581932}{WISEA J085039.98$+$441729.4} & $17$ & $.78$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.85$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3020$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.189$ & $\pm\,0.007$\rule{0pt}{3ex} & $5$ & $.5$ & $3$ & $.24$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_38_4_2__2.5934344165835532_0.0312168359736428}{WISEA J095422.27$+$014718.9} & $15$ & $.84$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.08$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $3650$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.10$\rule{0pt}{3ex} & $350$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.71712$ & $\pm\,0.00003$\rule{0pt}{3ex} & $9$ & $.8$ & $3$ & $.94$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_38_3_1__2.5961620441533730_0.0285885202472453}{WISEA J095459.77$+$013816.5} & $19$ & $.69$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.85$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $3010$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $620$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $23$ & $.11$ & $\pm\,0.09$\rule{0pt}{3ex} & $4$ & $.7$ & $1$ & $.39$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_67_4_0__2.6002941907360646_0.0504167121135645}{WISEA J095556.62$+$025319.1} & $18$ & $.00$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.89$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3640$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.09$\rule{0pt}{3ex} & $1100$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $10$ & $.72$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.42$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_47_3_3__2.6013758444276869_0.0363204835335277}{WISEA J095611.48$+$020451.5} & $15$ & $.37$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3300$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $170$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.1017$ & $\pm\,0.0008$\rule{0pt}{3ex} & $5$ & $.7$ & $5$ & $.75$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_46_4_0__2.6071237222958752_0.0361034418949703}{WISEA J095730.51$+$020407.0} & $18$ & $.98$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3090$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $560$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.441$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.5$ & $2$ & $.50$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_56_1_3__2.6088738440777850_0.0401060045814119}{WISEA J095754.58$+$021752.2} & $16$ & $.60$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $260$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.416$ & $\pm\,0.004$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.37$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_76_3_0__2.6093954159238040_0.0560698681010654}{WISEA J095801.76$+$031245.2} & $16$ & $.93$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $310$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $10$ & $.56$ & $\pm\,0.10$\rule{0pt}{3ex} & $5$ & $.4$ & $1$ & $.79$ & 33 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_76_1_3__2.6108307933335717_0.0531481514056822}{WISEA J095821.50$+$030242.6} & $17$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.97$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3600$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $660$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & P & $16$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.40$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_25_2_3__2.6115371561958383_0.0180923069298967}{WISEA J095831.20$+$010211.8} & $17$ & $.75$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3190$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $380$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.8220$ & $\pm\,0.0010$\rule{0pt}{3ex} & $1$ & $.6$ & $4$ & $.00$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_45_2_0__2.6123496057681339_0.0341443852199421}{WISEA J095842.37$+$015722.9} & $17$ & $.45$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.04$\rule{0pt}{3ex} & $3470$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $640$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $22$ & $.09$ & $\pm\,0.09$\rule{0pt}{3ex} & $2$ & $.3$ & $1$ & $.83$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_75_4_1__2.6135980414985274_0.0583633281496876}{WISEA J095859.54$+$032038.3} & $16$ & $.76$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3370$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.06$\rule{0pt}{3ex} & $410$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $42$ & $.4$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.70$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_45_4_2__2.6137014780339576_0.0373820436139074}{WISEA J095900.97$+$020830.5} & $16$ & $.78$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.92$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3610$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.08$\rule{0pt}{3ex} & $600$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.1793$ & $\pm\,0.0008$\rule{0pt}{3ex} & $2$ & $.3$ & $1$ & $.34$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_65_1_1__2.6149652852680139_0.0474385570640281}{WISEA J095918.34$+$024304.8} & $15$ & $.85$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3900$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.10$\rule{0pt}{3ex} & $550$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.4502$ & $\pm\,0.0004$\rule{0pt}{3ex} & $3$ & $.8$ & $2$ & $.82$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_75_3_0__2.6154283411780628_0.0585171485253294}{WISEA J095924.71$+$032109.9} & $17$ & $.73$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.99$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $2850$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.09$ & $\pm\,0.02$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.795$ & $\pm\,0.004$\rule{0pt}{3ex} & $5$ & $.6$ & $3$ & $.20$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_65_1_2__2.6156999048087077_0.0487531047808286}{WISEA J095928.43$+$024735.9} & $18$ & $.43$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3300$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $700$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $14$ & $.58$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.94$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_35_3_2__2.6167563258085882_0.0289281527967950}{WISEA J095942.97$+$013926.7} & $17$ & $.97$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $500$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.097$ & $\pm\,0.003$\rule{0pt}{3ex} & $2$ & $.6$ & $1$ & $.72$ & 28 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_75_3_3__2.6167747266425390_0.0574953909993375}{WISEA J095943.23$+$031739.3} & $18$ & $.68$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3110$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $490$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.886$ & $\pm\,0.004$\rule{0pt}{3ex} & $3$ & $.2$ & $4$ & $.91$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_14_4_3__2.6186065691830285_0.0161636529134954}{WISEA J100008.41$+$005534.2} & $18$ & $.22$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3440$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $800$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.637$ & $\pm\,0.005$\rule{0pt}{3ex} & $2$ & $.8$ & $3$ & $.49$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_14_2_1__2.6196430118469194_0.0126768243091379}{WISEA J100022.67$+$004334.6} & $18$ & $.38$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3170$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $480$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.2826$ & $\pm\,0.0007$\rule{0pt}{3ex} & $4$ & $.2$ & $2$ & $.66$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_84_2_3__2.6202904166656151_0.0606065716978627}{WISEA J100031.55$+$032820.9} & $17$ & $.41$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $320$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $21$ & $.79$ & $\pm\,0.10$\rule{0pt}{3ex} & $3$ & $.9$ & $1$ & $.96$ & 31 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_44_1_2__2.6218406391722602_0.0341034033536494}{WISEA J100052.90$+$015714.1} & $17$ & $.69$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.01$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $2860$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.10$ & $\pm\,0.02$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $23$ & $.61$ & $\pm\,0.10$\rule{0pt}{3ex} & $3$ & $.1$ & $1$ & $.52$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_43_4_1__2.6274155319573942_0.0370692156872000}{WISEA J100209.55$+$020725.8} & $17$ & $.79$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $11$ & $.19$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.31$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_22_2_3__2.6322655088469480_0.0201041667900320}{WISEA J100316.24$+$010905.8} & $17$ & $.50$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.94$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3590$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.46$ & $\pm\,0.09$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $7$ & $.236$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.88$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_72_2_3__2.6332287242215653_0.0529837640631495}{WISEA J100329.48$+$030208.4} & $17$ & $.14$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3850$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.10$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.740$ & $\pm\,0.002$\rule{0pt}{3ex} & $2$ & $.4$ & $3$ & $.00$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/4_31_4_1__2.6408869705366951_0.0279366957843490}{WISEA J100514.79$+$013602.2} & $16$ & $.37$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.95$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3570$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $490$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.342$ & $\pm\,0.007$\rule{0pt}{3ex} & $1$ & $.7$ & $2$ & $.29$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_77_2_2__2.7870406891617754_1.0282997038553159}{WISEA J103844.55$+$585501.9} & $16$ & $.87$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.01$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3490$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $540$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $29$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.37$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_27_2_3__2.7905749593888380_0.9936939486141497}{WISEA J103933.15$+$565604.1} & $17$ & $.01$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $3300$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $320$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $27$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & $6$ & $.1$ & $1$ & $.74$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_37_3_1__2.7986808559670004_1.0057753375537370}{WISEA J104124.61$+$573736.0} & $17$ & $.49$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3110$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $270$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $17$ & $.46$ & $\pm\,0.07$\rule{0pt}{3ex} & $3$ & $.5$ & $1$ & $.39$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_36_2_2__2.8011221439396183_1.0024666383392735}{WISEA J104158.19$+$572613.6} & $16$ & $.98$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3500$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $490$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $56$ & $.3$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.16$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_76_4_2__2.8043230733625673_1.0328038245605105}{WISEA J104242.21$+$591030.7} & $17$ & $.76$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3170$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $360$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $91$ &  & $\pm\,2$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.01$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_46_3_2__2.8072873751589662_1.0125634634881624}{WISEA J104322.98$+$580056.1} & $15$ & $.68$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3740$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.10$\rule{0pt}{3ex} & $440$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $11$ & $.40$ & $\pm\,0.03$\rule{0pt}{3ex} & $5$ & $.8$ & $1$ & $.22$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_46_3_3__2.8086001754270349_1.0113833446865972}{WISEA J104341.02$+$575652.8} & $16$ & $.52$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.89$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3480$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.07$\rule{0pt}{3ex} & $420$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.8190$ & $\pm\,0.0004$\rule{0pt}{3ex} & $5$ & $.2$ & $2$ & $.34$ & 59 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_86_1_2__2.8116810861114212_1.0378413635187556}{WISEA J104423.39$+$592750.0} & $16$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $3850$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.10$\rule{0pt}{3ex} & $640$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $7$ & $.171$ & $\pm\,0.009$\rule{0pt}{3ex} & $3$ & $.4$ & $1$ & $.80$ & 35 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_15_4_2__2.8133912811561568_0.9915282575122391}{WISEA J104446.91$+$564837.0} & $18$ & $.93$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3320$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $24$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.51$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_65_2_1__2.8143574658759687_1.0233045350322678}{WISEA J104500.17$+$583751.6} & $17$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3440$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.07$\rule{0pt}{3ex} & $560$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $13$ & $.10$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.65$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_85_2_1__2.8173851051530652_1.0357616745568667}{WISEA J104541.81$+$592041.1} & $16$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3120$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $30$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & $3$ & $.7$ & $1$ & $.68$ & 38 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_25_1_1__2.8204880459183825_0.9951751074114984}{WISEA J104624.48$+$570109.6} & $16$ & $.81$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.84$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3700$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.09$\rule{0pt}{3ex} & $690$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.04$ & $\pm\,0.03$\rule{0pt}{3ex} & $2$ & $.7$ & $1$ & $.90$ & 33 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_55_3_3__2.8205409673581694_1.0178288575998933}{WISEA J104625.20$+$581902.1} & $18$ & $.31$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.07$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3570$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.09$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.562$ & $\pm\,0.004$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.17$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_65_1_1__2.8208735950807604_1.0211778395747280}{WISEA J104629.79$+$583033.1} & $16$ & $.90$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3330$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $340$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $18$ & $.54$ & $\pm\,0.08$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.69$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_35_3_3__2.8211711468226359_1.0067821359280136}{WISEA J104633.88$+$574103.6} & $15$ & $.95$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3320$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $240$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $8$ & $.77$ & $\pm\,0.02$\rule{0pt}{3ex} & $2$ & $.4$ & $3$ & $.23$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_65_1_3__2.8219655881478429_1.0237413012612204}{WISEA J104644.83$+$583921.6} & $18$ & $.06$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $99$ &  & $\pm\,3$\rule{0pt}{3ex} & $2$ & $.6$ & $1$ & $.01$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_45_1_1__2.8227562177794288_1.0094442227123626}{WISEA J104655.68$+$575012.7} & $16$ & $.33$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3320$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.4793$ & $\pm\,0.0010$\rule{0pt}{3ex} & $1$ & $.3$ & $1$ & $.72$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_55_3_3__2.8233208207575871_1.0198337300595639}{WISEA J104703.46$+$582555.8} & $17$ & $.92$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3320$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $550$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $68$ & $.8$ & $\pm\,1.0$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.07$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_14_4_2__2.8272343252568057_0.9899055111651111}{WISEA J104757.25$+$564302.5} & $16$ & $.90$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.87$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.84$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $3020$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $180$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $86$ &  & $\pm\,2$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.01$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_24_2_1__2.8314451941444863_0.9928412020869847}{WISEA J104855.15$+$565308.2} & $17$ & $.81$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.89$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.91$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $2960$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.12$ & $\pm\,0.02$\rule{0pt}{3ex} & $220$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.7974$ & $\pm\,0.0004$\rule{0pt}{3ex} & $6$ & $.6$ & $4$ & $.50$ & 56 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_24_4_2__2.8319725687336468_0.9993835576194188}{WISEA J104902.43$+$571537.5} & $18$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3370$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $630$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.3426$ & $\pm\,0.0010$\rule{0pt}{3ex} & $4$ & $.6$ & $9$ & $.59$ & 49 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_14_3_2__2.8324494001111509_0.9918631382097886}{WISEA J104908.96$+$564946.4} & $16$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.96$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3620$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.09$\rule{0pt}{3ex} & $480$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $41$ & $.0$ & $\pm\,1.0$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.59$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_34_3_1__2.8351570075355106_1.0036942723932047}{WISEA J104946.22$+$573026.7} & $17$ & $.49$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $390$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7239$ & $\pm\,0.0002$\rule{0pt}{3ex} & $4$ & $.7$ & $2$ & $.00$ & 73 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_74_1_2__2.8361405425192174_1.0295467870900845}{WISEA J104959.75$+$585919.1} & $18$ & $.25$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.09$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3500$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.08$\rule{0pt}{3ex} & $1000$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.8398$ & $\pm\,0.0002$\rule{0pt}{3ex} & $3$ & $.2$ & $1$ & $.61$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_33_2_3__2.8427353956046906_1.0013292886147431}{WISEA J105130.40$+$572218.9} & $16$ & $.63$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3510$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.08$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.313$ & $\pm\,0.002$\rule{0pt}{3ex} & $3$ & $.7$ & $1$ & $.13$ & 45 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_73_1_1__2.8497706944441807_1.0296438077516157}{WISEA J105307.14$+$585939.3} & $18$ & $.53$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3100$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.03$\rule{0pt}{3ex} & $460$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $36$ & $.0$ & $\pm\,0.3$\rule{0pt}{3ex} & $3$ & $.2$ & $1$ & $.68$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_32_2_1__2.8555571878693713_1.0008043333531900}{WISEA J105426.72$+$572030.5} & $17$ & $.48$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.94$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3690$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.10$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $39$ & $.3$ & $\pm\,0.4$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.48$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_42_1_0__2.8647882577078820_1.0067374949111534}{WISEA J105633.65$+$574054.5} & $17$ & $.05$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.87$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3610$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.08$\rule{0pt}{3ex} & $700$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.8020$ & $\pm\,0.0010$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.92$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_61_2_3__2.8693946764057228_1.0214606991464072}{WISEA J105736.95$+$583131.8} & $18$ & $.03$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $540$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.7079$ & $\pm\,0.0002$\rule{0pt}{3ex} & $3$ & $.6$ & $3$ & $.96$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/5_41_3_3__2.8722138889444171_1.0111204391623501}{WISEA J105815.77$+$575558.5} & $17$ & $.60$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3130$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.04$\rule{0pt}{3ex} & $330$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $31$ & $.3$ & $\pm\,0.3$\rule{0pt}{3ex} & $3$ & $.4$ & $1$ & $.45$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_38_1_0__3.1971502051565888_0.8109031667143716}{WISEA J121243.98$+$462741.1} & $18$ & $.84$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $550$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.5446$ & $\pm\,0.0008$\rule{0pt}{3ex} & $6$ & $.1$ & $2$ & $.04$ & 40 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_38_3_2__3.1978736120788867_0.8147786451537880}{WISEA J121253.93$+$464100.2} & $16$ & $.41$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $230$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.2980$ & $\pm\,0.0010$\rule{0pt}{3ex} & $2$ & $.4$ & $7$ & $.31$ & 28 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_57_1_3__3.2046932590710275_0.8227324748990321}{WISEA J121427.69$+$470820.6} & $16$ & $.37$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.91$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3610$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.09$\rule{0pt}{3ex} & $500$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.8276$ & $\pm\,0.0005$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.15$ & 42 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_27_3_0__3.2075361309512127_0.8051462007749309}{WISEA J121506.78$+$460753.2} & $16$ & $.46$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3190$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $210$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $91$ &  & $\pm\,2$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.02$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_26_1_1__3.2176628511543957_0.8016566896593946}{WISEA J121726.04$+$455553.4} & $15$ & $.69$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & $0$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3360$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $220$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.8802$ & $\pm\,0.0002$\rule{0pt}{3ex} & $1$ & $.7$ & $1$ & $.73$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_25_4_2__3.2215117548125596_0.8062230245707748}{WISEA J121818.97$+$461134.9} & $18$ & $.39$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3360$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.06$\rule{0pt}{3ex} & $700$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $13$ & $.6920$ & $\pm\,0.0010$\rule{0pt}{3ex} & $3$ & $.1$ & $2$ & $.02$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_65_1_1__3.2252337072504433_0.8328452406681561}{WISEA J121910.13$+$474306.6} & $16$ & $.46$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3150$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.04$\rule{0pt}{3ex} & $200$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $13$ & $.69$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.68$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_45_3_1__3.2257870012403149_0.8206220729469619}{WISEA J121917.75$+$470105.2} & $15$ & $.91$ & $\pm\,0.04$\rule{0pt}{3ex} & $0$ & $.93$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.08$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3670$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.10$\rule{0pt}{3ex} & $270$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $55$ & $.0$ & $\pm\,0.6$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.15$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_85_1_0__3.2271761698517532_0.8461207812445803}{WISEA J121936.85$+$482844.7} & $16$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3090$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.03$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.8864$ & $\pm\,0.0007$\rule{0pt}{3ex} & $3$ & $.6$ & $2$ & $.73$ & 38 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_84_2_1__3.2299331660144972_0.8461109555872021}{WISEA J122014.75$+$482842.8} & $16$ & $.63$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3440$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.08$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $52$ & $.3$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.3$ & $1$ & $.22$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_64_2_0__3.2328374680132250_0.8302058394382721}{WISEA J122054.67$+$473402.0} & $18$ & $.39$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $560$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $83$ & $.8$ & $\pm\,1.0$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.02$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_24_3_2__3.2369543121493636_0.8079271171093777}{WISEA J122151.32$+$461726.9} & $15$ & $.81$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.84$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.05$\rule{0pt}{3ex} & $3040$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $110$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.87060$ & $\pm\,0.00010$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.65$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_53_4_2__3.2435802408457546_0.8274043239668825}{WISEA J122322.42$+$472424.4} & $18$ & $.41$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3080$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $420$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $10$ & $.24$ & $\pm\,0.02$\rule{0pt}{3ex} & $2$ & $.0$ & $3$ & $.61$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_32_2_0__3.2508557370872202_0.8112118612304400}{WISEA J122502.46$+$462844.3} & $17$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.06$\rule{0pt}{3ex} & $3870$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.10$\rule{0pt}{3ex} & $1200$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.8332$ & $\pm\,0.0004$\rule{0pt}{3ex} & $3$ & $.6$ & $1$ & $.14$ & 34 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_42_2_2__3.2526192571431713_0.8168560252782576}{WISEA J122526.71$+$464808.7} & $18$ & $.50$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3150$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.04$\rule{0pt}{3ex} & $510$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $6$ & $.95$ & $\pm\,0.02$\rule{0pt}{3ex} & $3$ & $.7$ & $6$ & $.66$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_52_4_1__3.2543805330944591_0.8288242406818631}{WISEA J122550.94$+$472917.2} & $17$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3620$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.08$\rule{0pt}{3ex} & $700$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1453$ & $\pm\,0.0009$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.39$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/6_51_4_0__3.2633894739914964_0.8262434471323543}{WISEA J122754.82$+$472024.8} & $17$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3370$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.06$\rule{0pt}{3ex} & $440$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.2750$ & $\pm\,0.0006$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.51$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_56_4_0__3.7058210495008757_0.9348034732611868}{WISEA J140918.68$+$533337.2} & $19$ & $.02$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $560$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.80104$ & $\pm\,0.00005$\rule{0pt}{3ex} & $3$ & $.9$ & $2$ & $.04$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_36_1_1__3.7099050001087517_0.9154755042326007}{WISEA J141014.83$+$522710.7} & $18$ & $.20$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3400$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.07$\rule{0pt}{3ex} & $700$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $16$ & $.86$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.67$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_26_3_1__3.7105003342797418_0.9132894908122533}{WISEA J141023.05$+$521939.4} & $18$ & $.28$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.94$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.95$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.05$\rule{0pt}{3ex} & $2950$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.13$ & $\pm\,0.02$\rule{0pt}{3ex} & $260$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $15$ & $.8$ & $\pm\,0.3$\rule{0pt}{3ex} & $4$ & $.3$ & $1$ & $.95$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_56_1_0__3.7116002643140669_0.9296512464937080}{WISEA J141038.13$+$531554.0} & $18$ & $.86$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.01$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3550$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $1400$ &  & $\pm\,300$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.1336$ & $\pm\,0.0010$\rule{0pt}{3ex} & $3$ & $.2$ & $2$ & $.33$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_76_1_3__3.7132472528486589_0.9466989874855751}{WISEA J141100.79$+$541430.7} & $17$ & $.58$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3490$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $610$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $84$ & $.9$ & $\pm\,1.0$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.03$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_45_2_1__3.7155038765182211_0.9249221402875453}{WISEA J141131.82$+$525938.7} & $19$ & $.19$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.84$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $3030$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.03$\rule{0pt}{3ex} & $510$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.824$ & $\pm\,0.002$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.53$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_35_2_0__3.7163827921007200_0.9155868751902395}{WISEA J141143.93$+$522733.2} & $15$ & $.88$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3280$ &  & $\pm\,90$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $210$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3474$ & $\pm\,0.0006$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.94$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_65_4_1__3.7169559092822526_0.9409601336215768}{WISEA J141151.81$+$535446.8} & $16$ & $.68$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3410$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $360$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $62$ & $.4$ & $\pm\,0.7$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.06$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_65_2_3__3.7170089409395781_0.9372402767162147}{WISEA J141152.54$+$534159.5} & $18$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.81$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $3080$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $380$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $129$ &  & $\pm\,3$\rule{0pt}{3ex} & $3$ & $.1$ & $1$ & $.01$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_55_3_2__3.7207528129635659_0.9338591629236446}{WISEA J141243.99$+$533022.6} & $17$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $300$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $35$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.74$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_55_3_1__3.7218950235392256_0.9329706028066431}{WISEA J141259.72$+$532719.1} & $17$ & $.38$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.81$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $3730$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7315$ & $\pm\,0.0002$\rule{0pt}{3ex} & $6$ & $.0$ & $2$ & $.07$ & 45 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_25_1_2__3.7220404175270363_0.9104344128856580}{WISEA J141301.71$+$520950.5} & $17$ & $.36$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3340$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.06$\rule{0pt}{3ex} & $450$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $99$ &  & $\pm\,4$\rule{0pt}{3ex} & $1$ & $.3$ & $1$ & $.01$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_25_1_1__3.7227702193484054_0.9104579831181288}{WISEA J141311.74$+$520955.3} & $15$ & $.90$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3430$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.07$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1725$ & $\pm\,0.0010$\rule{0pt}{3ex} & $1$ & $.8$ & $2$ & $.28$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_35_3_1__3.7239206243413827_0.9216874509261050}{WISEA J141327.57$+$524831.6} & $16$ & $.08$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.04$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.96$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $2900$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.10$ & $\pm\,0.02$\rule{0pt}{3ex} & $90$ &  & $\pm\,20$\rule{0pt}{3ex} & $-2$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7711$ & $\pm\,0.0002$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.65$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_14_1_1__3.7349193789562167_0.9028413042558321}{WISEA J141558.82$+$514345.1} & $17$ & $.84$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3280$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.6787$ & $\pm\,0.0010$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.34$ & 26 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_74_1_1__3.7373099421974731_0.9456005086629355}{WISEA J141631.71$+$541044.2} & $18$ & $.22$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.10$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.08$\rule{0pt}{3ex} & $760$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $4$ & $.267$ & $\pm\,0.008$\rule{0pt}{3ex} & $2$ & $.2$ & $2$ & $.94$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_33_1_0__3.7453124482164921_0.9162756196398609}{WISEA J141821.72$+$522955.2} & $17$ & $.50$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3100$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.03$\rule{0pt}{3ex} & $270$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.5997$ & $\pm\,0.0005$\rule{0pt}{3ex} & $1$ & $.8$ & $3$ & $.88$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/7_32_4_1__3.7502456640734230_0.9192733858777935}{WISEA J141929.58$+$524013.8} & $16$ & $.21$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3500$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.08$\rule{0pt}{3ex} & $340$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $63$ & $.2$ & $\pm\,0.8$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.06$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_67_2_0__4.2025101664607627_0.9677654966060996}{WISEA J160308.66$+$552655.9} & $17$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3130$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $290$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.79413$ & $\pm\,0.00010$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.24$ & 35 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_67_4_2__4.2026836514527419_0.9706106950611616}{WISEA J160311.02$+$553642.6} & $19$ & $.20$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3130$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.04$\rule{0pt}{3ex} & $640$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $6$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $3$ & $.9$ & $4$ & $.13$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_37_2_1__4.2030810161639156_0.9471160184431993}{WISEA J160316.52$+$541556.7} & $18$ & $.57$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $2$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $2720$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.084$ & $\pm\,0.010$\rule{0pt}{3ex} & $180$ &  & $\pm\,40$\rule{0pt}{3ex} & $-3$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $98$ &  & $\pm\,2$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.01$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_27_3_3__4.2089703360080666_0.9431537227735919}{WISEA J160437.49$+$540219.6} & $15$ & $.79$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.00$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3560$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.08$\rule{0pt}{3ex} & $330$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.8034$ & $\pm\,0.0003$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.99$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_67_3_2__4.2105497466302682_0.9717226537321901}{SDSS J160459.21$+$554032.1} & $19$ & $.77$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3360$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $1500$ &  & $\pm\,300$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $6$ & $.252$ & $\pm\,0.007$\rule{0pt}{3ex} & $7$ & $.4$ & $5$ & $.75$ & 45 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_57_1_2__4.2109117847065338_0.9602799090443340}{WISEA J160504.36$+$550111.3} & $18$ & $.32$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $3900$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.10$\rule{0pt}{3ex} & $1700$ &  & $\pm\,300$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.8092$ & $\pm\,0.0007$\rule{0pt}{3ex} & $3$ & $.4$ & $1$ & $.30$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_27_1_1__4.2119502702888543_0.9394491908383804}{WISEA J160518.46$+$534935.4} & $18$ & $.64$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3030$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $410$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $3$ & $.614$ & $\pm\,0.010$\rule{0pt}{3ex} & $12$ & $.5$ & $2$ & $.06$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_27_1_0__4.2135295009488809_0.9403326767266648}{WISEA J160540.16$+$535237.8} & $19$ & $.00$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3120$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $600$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $128$ &  & $\pm\,3$\rule{0pt}{3ex} & $2$ & $.9$ & $1$ & $.01$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_36_4_2__4.2153806279533983_0.9501583764404422}{WISEA J160605.64$+$542624.1} & $17$ & $.11$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3220$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $310$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $12$ & $.74$ & $\pm\,0.03$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.59$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_46_3_2__4.2206814299698312_0.9574196479664552}{WISEA J160718.52$+$545121.8} & $16$ & $.82$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.09$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3820$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.10$\rule{0pt}{3ex} & $730$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.161$ & $\pm\,0.010$\rule{0pt}{3ex} & $3$ & $.3$ & $4$ & $.01$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_66_3_2__4.2223475093982250_0.9701501161937466}{WISEA J160741.43$+$553507.8} & $18$ & $.37$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $450$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $14$ & $.26$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.7$ & $1$ & $.02$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_16_1_2__4.2228652785831127_0.9339541046187169}{WISEA J160748.56$+$533041.8} & $16$ & $.83$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.652$ & $\pm\,0.002$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.08$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_86_1_1__4.2237503079657905_0.9834757477465393}{WISEA J160800.73$+$562056.5} & $15$ & $.82$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.07$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.01$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3690$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.10$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.190$ & $\pm\,0.005$\rule{0pt}{3ex} & $2$ & $.9$ & $2$ & $.79$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_56_3_2__4.2237925692533951_0.9636259142331767}{WISEA J160801.31$+$551242.0} & $17$ & $.08$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.97$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3630$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $710$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $47$ & $.8$ & $\pm\,0.4$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.23$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_65_4_0__4.2256396142211425_0.9699351723991748}{WISEA J160826.71$+$553423.4} & $15$ & $.76$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $3240$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $180$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.2240$ & $\pm\,0.0007$\rule{0pt}{3ex} & $4$ & $.1$ & $1$ & $.88$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_65_4_2__4.2264204935649072_0.9698517172521546}{WISEA J160837.44$+$553406.3} & $16$ & $.79$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.97$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3620$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $580$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.5496$ & $\pm\,0.0007$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.92$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_15_4_3__4.2267338181028355_0.9379552648525249}{WISEA J160841.74$+$534427.3} & $16$ & $.52$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3470$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.07$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $24$ & $.8$ & $\pm\,0.7$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.30$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_75_2_0__4.2270228406199273_0.9752552802822588}{WISEA J160845.72$+$555240.7} & $15$ & $.70$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $220$ &  & $\pm\,40$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $14$ & $.44$ & $\pm\,0.03$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.34$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_75_4_1__4.2278989490165060_0.9780927746148794}{WISEA J160857.77$+$560226.2} & $17$ & $.29$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.92$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $3700$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $43$ & $.1$ & $\pm\,0.4$\rule{0pt}{3ex} & $1$ & $.1$ & $1$ & $.25$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_55_2_1__4.2303444723242967_0.9604839302157269}{WISEA J160931.39$+$550154.1} & $17$ & $.83$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3230$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $430$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.8952$ & $\pm\,0.0002$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.75$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_65_2_0__4.2311907986845227_0.9669293668729239}{WISEA J160943.07$+$552403.5} & $18$ & $.00$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3360$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $670$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $7$ & $.82$ & $\pm\,0.07$\rule{0pt}{3ex} & $3$ & $.6$ & $4$ & $.21$ & 20 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_25_3_1__4.2318736216886510_0.9451059650891622}{WISEA J160952.45$+$540902.0} & $17$ & $.70$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.02$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3590$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.09$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $42$ & $.3$ & $\pm\,0.5$\rule{0pt}{3ex} & $1$ & $.7$ & $1$ & $.28$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_45_1_2__4.2321359562934306_0.9531774309298037}{WISEA J160956.04$+$543646.9} & $17$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $48$ & $.6$ & $\pm\,0.4$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.30$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_75_3_0__4.2364695141168900_0.9793777690408083}{WISEA J161055.63$+$560651.1} & $18$ & $.96$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.178$ & $\pm\,0.003$\rule{0pt}{3ex} & $10$ & $.4$ & $1$ & $.46$ & 56 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_34_2_0__4.2377298599755742_0.9468820305207538}{WISEA J161112.96$+$541508.3} & $17$ & $.62$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $390$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $15$ & $.14$ & $\pm\,0.04$\rule{0pt}{3ex} & $3$ & $.0$ & $1$ & $.07$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_74_4_2__4.2386315476631626_0.9773336154970873}{WISEA J161125.37$+$555949.7} & $18$ & $.25$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.62$ & $\pm\,0.04$\rule{0pt}{3ex} & $0$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $440$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $17$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.35$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_14_4_2__4.2398239906337309_0.9356377881849380}{WISEA J161141.76$+$533629.2} & $17$ & $.03$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.82$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $3050$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $210$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.881$ & $\pm\,0.007$\rule{0pt}{3ex} & $1$ & $.3$ & $6$ & $.22$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_34_3_2__4.2492687798680109_0.9509257567248235}{WISEA J161351.66$+$542902.4} & $17$ & $.40$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3480$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.08$\rule{0pt}{3ex} & $580$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.046$ & $\pm\,0.003$\rule{0pt}{3ex} & $3$ & $.1$ & $14$ & $.13$ & 41 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_64_1_1__4.2495871936200391_0.9689093721702642}{WISEA J161356.01$+$553051.9} & $16$ & $.02$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.57$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.76$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3150$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.04$\rule{0pt}{3ex} & $150$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.577$ & $\pm\,0.003$\rule{0pt}{3ex} & $1$ & $.4$ & $2$ & $.11$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_84_1_3__4.2498303847902763_0.9799943755817774}{WISEA J161359.36$+$560858.3} & $17$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3350$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $410$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7375$ & $\pm\,0.0008$\rule{0pt}{3ex} & $1$ & $.9$ & $2$ & $.05$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_13_4_3__4.2533148370541678_0.9361608622673708}{WISEA J161447.28$+$533817.0} & $16$ & $.92$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.48$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3200$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.04$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $50$ & $.3$ & $\pm\,0.7$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.13$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_53_2_2__4.2541919506281358_0.9612676072312351}{WISEA J161459.34$+$550435.6} & $16$ & $.10$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.06$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3590$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.48$ & $\pm\,0.09$\rule{0pt}{3ex} & $410$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $35$ & $.3$ & $\pm\,0.5$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.53$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_33_1_3__4.2593115022576082_0.9468003243123021}{WISEA J161609.74$+$541451.5} & $17$ & $.69$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.07$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $3860$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.10$\rule{0pt}{3ex} & $1100$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.0527$ & $\pm\,0.0008$\rule{0pt}{3ex} & $5$ & $.7$ & $1$ & $.69$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_73_3_3__4.2612470611089810_0.9768656652826019}{WISEA J161636.35$+$555813.0} & $16$ & $.55$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.95$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $3590$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.49$ & $\pm\,0.09$\rule{0pt}{3ex} & $500$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $41$ & $.2$ & $\pm\,0.8$\rule{0pt}{3ex} & $1$ & $.4$ & $1$ & $.39$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_42_2_1__4.2645042739779404_0.9520522515294322}{WISEA J161721.13$+$543254.8} & $17$ & $.34$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.55$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.08$\rule{0pt}{3ex} & $550$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.670$ & $\pm\,0.005$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.48$ & 33 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_52_4_3__4.2662225938662734_0.9628531441872733}{WISEA J161744.75$+$551002.7} & $18$ & $.02$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3110$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $380$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $39$ & $.7$ & $\pm\,0.4$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.19$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_72_2_1__4.2674086917643361_0.9745792992977830}{WISEA J161801.07$+$555021.4} & $17$ & $.07$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3240$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $25$ & $.99$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.7$ & $1$ & $.86$ & 28 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_52_1_2__4.2699365368455542_0.9601138979704901}{WISEA J161835.83$+$550037.6} & $17$ & $.49$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3380$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $55$ & $.07$ & $\pm\,0.02$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.14$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/8_51_4_1__4.2774082430521565_0.9654282046480622}{WISEA J162018.58$+$551853.9} & $16$ & $.41$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.14$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3420$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $330$ &  & $\pm\,60$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $64$ & $.0$ & $\pm\,0.7$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.05$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_58_1_0__5.8072459420314342_0.0056985511168818}{WISEA J221055.36$+$001935.4} & $15$ & $.69$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.7158$ & $\pm\,0.0009$\rule{0pt}{3ex} & $4$ & $.7$ & $3$ & $.83$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_67_3_2__5.8124053954513126_0.0154768965712010}{WISEA J221206.31$+$005312.2} & $17$ & $.50$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $390$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $64$ & $.0$ & $\pm\,1.0$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.07$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_67_1_1__5.8132781047751747_0.0128685075948150}{WISEA J221218.31$+$004414.1} & $17$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3440$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.07$\rule{0pt}{3ex} & $510$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $49$ & $.3$ & $\pm\,0.5$\rule{0pt}{3ex} & $1$ & $.1$ & $1$ & $.25$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_67_3_1__5.8134375075917797_0.0171825098520260}{WISEA J221220.49$+$005904.1} & $17$ & $.14$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $3310$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $360$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3506$ & $\pm\,0.0008$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.60$ & 31 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_37_3_3__5.8142957978420178_-0.0053512486698590}{WISEA J221232.29$-$001824.0} & $18$ & $.78$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.91$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.89$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $2970$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.13$ & $\pm\,0.02$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $38$ & $.2$ & $\pm\,0.3$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.18$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_36_4_1__5.8168001736891224_-0.0038438683679024}{WISEA J221306.75$-$001313.0} & $16$ & $.79$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $3830$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.10$\rule{0pt}{3ex} & $800$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & P & $30$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & $1$ & $.2$ & $1$ & $.64$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_76_2_3__5.8176056013082142_0.0200786272498173}{WISEA J221317.82$+$010901.3} & $17$ & $.19$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3830$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.10$\rule{0pt}{3ex} & $1000$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.891$ & $\pm\,0.002$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.93$ & 29 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_35_2_3__5.8230754511037830_-0.0080764148700398}{WISEA J221433.03$-$002745.8} & $16$ & $.34$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.09$\rule{0pt}{3ex} & $1$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.06$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $10$ & $.15$ & $\pm\,0.08$\rule{0pt}{3ex} & $2$ & $.4$ & $3$ & $.48$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_65_2_1__5.8239677738898825_0.0130965547394138}{WISEA J221445.29$+$004500.7} & $20$ & $.57$ & $\pm\,0.04$\rule{0pt}{3ex} & \multicolumn{3}{c}{}\rule{0pt}{3ex} & $2$ & $.56$ & $\pm\,0.10$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $2990$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-3$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.0756$ & $\pm\,0.0006$\rule{0pt}{3ex} & $10$ & $.9$ & $8$ & $.68$ & 26 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_25_4_1__5.8250162494499582_-0.0102893420635152}{WISEA J221459.70$-$003522.6} & $18$ & $.08$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.88$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $3650$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.09$\rule{0pt}{3ex} & $1200$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $9$ & $.69$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.0$ & $2$ & $.27$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_65_1_1__5.8257175317886167_0.0127868963514199}{WISEA J221509.36$+$004357.4} & $16$ & $.51$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.82$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $3050$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1948$ & $\pm\,0.0002$\rule{0pt}{3ex} & $2$ & $.0$ & $4$ & $.04$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_15_3_1__5.8257642675270818_-0.0178263136641073}{WISEA J221509.99$-$010116.9} & $17$ & $.29$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.43$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $8$ & $.606$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.82$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_25_1_3__5.8259991853241528_-0.0141046510775342}{WISEA J221513.23$-$004829.3} & $16$ & $.04$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3640$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.51$ & $\pm\,0.09$\rule{0pt}{3ex} & $420$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.372$ & $\pm\,0.004$\rule{0pt}{3ex} & $3$ & $.5$ & $1$ & $.25$ & 38 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_45_1_0__5.8260037087941496_0.0001166318090948}{WISEA J221513.30$+$000024.1} & $17$ & $.68$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3410$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $630$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $53$ &  & $\pm\,3$\rule{0pt}{3ex} & $2$ & $.0$ & $1$ & $.21$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_45_3_3__5.8261848513551238_0.0045172653766716}{WISEA J221515.79$+$001531.3} & $18$ & $.37$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.08$\rule{0pt}{3ex} & $1$ & $.38$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3290$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $650$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.80150$ & $\pm\,0.00008$\rule{0pt}{3ex} & $7$ & $.6$ & $3$ & $.38$ & 45 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_45_3_2__5.8275697750418631_0.0019908373091153}{WISEA J221534.82$+$000650.6} & $16$ & $.61$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.91$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.46$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3560$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $530$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $39$ & $.9$ & $\pm\,0.3$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.13$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_35_3_3__5.8281894965544083_-0.0047885796128064}{WISEA J221543.35$-$001627.6} & $16$ & $.70$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.09$\rule{0pt}{3ex} & $1$ & $.44$ & $\pm\,0.08$\rule{0pt}{3ex} & $0$ & $.69$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $3220$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $270$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.825$ & $\pm\,0.006$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.71$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_25_1_1__5.8282664353727514_-0.0150706170841435}{WISEA J221544.41$-$005148.5} & $17$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.10$\rule{0pt}{3ex} & $1$ & $.56$ & $\pm\,0.09$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.07$\rule{0pt}{3ex} & $3170$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $380$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $28$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & $2$ & $.4$ & $1$ & $.24$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_24_4_1__5.8290517510796898_-0.0102726583113167}{WISEA J221555.21$-$003518.7} & $18$ & $.05$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.08$\rule{0pt}{3ex} & $1$ & $.65$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3090$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $370$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.2540$ & $\pm\,0.0003$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.76$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_64_4_0__5.8321036800302801_0.0177937373905179}{WISEA J221637.18$+$010110.0} & $17$ & $.16$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.95$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3580$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.47$ & $\pm\,0.09$\rule{0pt}{3ex} & $680$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.57$ & $\pm\,0.03$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.72$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_84_1_0__5.8337747615940208_0.0287921100660885}{WISEA J221700.16$+$013858.6} & $16$ & $.03$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3340$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.277$ & $\pm\,0.008$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.75$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_84_1_2__5.8345990337070344_0.0272601687915122}{WISEA J221711.50$+$013342.8} & $17$ & $.22$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $3100$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $240$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $48$ & $.9$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.15$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_14_3_2__5.8350316497007926_-0.0169429999659333}{WISEA J221717.42$-$005814.1} & $18$ & $.44$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.90$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $3630$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.51$ & $\pm\,0.09$\rule{0pt}{3ex} & $1200$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.438$ & $\pm\,0.005$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.77$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_34_1_0__5.8353750752107851_-0.0077216731043379}{WISEA J221722.17$-$002632.9} & $17$ & $.56$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.05$ & $\pm\,0.09$\rule{0pt}{3ex} & $1$ & $.01$ & $\pm\,0.08$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.07$\rule{0pt}{3ex} & $2850$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.09$ & $\pm\,0.02$\rule{0pt}{3ex} & $150$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.401$ & $\pm\,0.003$\rule{0pt}{3ex} & $5$ & $.2$ & $3$ & $.09$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_64_3_0__5.8358436382363310_0.0158702120391042}{SDSS J221728.62$+$005433.4} & $18$ & $.94$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.54$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $720$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.1949$ & $\pm\,0.0010$\rule{0pt}{3ex} & $6$ & $.1$ & $5$ & $.52$ & 25 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_43_2_3__5.8377341859256191_-0.0004150921707587}{WISEA J221754.61$-$000125.8} & $17$ & $.08$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.98$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3510$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.43$ & $\pm\,0.08$\rule{0pt}{3ex} & $580$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.239$ & $\pm\,0.007$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.27$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_53_3_2__5.8405694688249925_0.0093051428019279}{WISEA J221833.59$+$003159.2} & $17$ & $.71$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3160$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $340$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $22$ & $.95$ & $\pm\,0.10$\rule{0pt}{3ex} & $2$ & $.3$ & $1$ & $.63$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_33_1_3__5.8411768585708383_-0.0083221973468518}{WISEA J221841.94$-$002836.6} & $16$ & $.61$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3670$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.51$ & $\pm\,0.09$\rule{0pt}{3ex} & $620$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.80558$ & $\pm\,0.00010$\rule{0pt}{3ex} & $2$ & $.8$ & $1$ & $.46$ & 22 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_23_3_0__5.8414272180750508_-0.0092484752909303}{WISEA J221845.40$-$003147.8} & $17$ & $.60$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.87$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.05$\rule{0pt}{3ex} & $3570$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $900$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.6318$ & $\pm\,0.0010$\rule{0pt}{3ex} & $2$ & $.1$ & $7$ & $.42$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_13_3_2__5.8421283828514072_-0.0170975617267856}{WISEA J221855.03$-$005846.7} & $17$ & $.61$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3980$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.10$\rule{0pt}{3ex} & $1400$ &  & $\pm\,300$\rule{0pt}{3ex} & $-1$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $7$ & $.978$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.4$ & $2$ & $.84$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_42_4_0__5.8433032029688201_0.0015227448351773}{WISEA J221911.19$+$000513.9} & $16$ & $.05$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.42$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.61$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3360$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.07$\rule{0pt}{3ex} & $250$ &  & $\pm\,50$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3502$ & $\pm\,0.0004$\rule{0pt}{3ex} & $2$ & $.0$ & $2$ & $.26$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_72_1_1__5.8466680951421264_0.0196296511415524}{WISEA J221957.46$+$010728.8} & $15$ & $.54$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.22$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.42$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3650$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.09$\rule{0pt}{3ex} & $370$ &  & $\pm\,70$\rule{0pt}{3ex} & $-1$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.247$ & $\pm\,0.003$\rule{0pt}{3ex} & $2$ & $.7$ & $1$ & $.62$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_22_3_1__5.8477909351602451_-0.0100312030936218}{WISEA J222012.89$-$003429.1} & $15$ & $.55$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.04$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.53$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $3980$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.74$ & $\pm\,0.10$\rule{0pt}{3ex} & $470$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $2$ & $.7655$ & $\pm\,0.0010$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.70$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_42_3_1__5.8480179599530162_0.0046518733231540}{WISEA J222016.02$+$001559.3} & $16$ & $.07$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.42$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.67$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3250$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $210$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $31$ & $.643$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.58$ & 23 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_61_4_3__5.8513644533491105_0.0185991348505162}{WISEA J222102.06$+$010356.4} & $16$ & $.68$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.34$ & $\pm\,0.09$\rule{0pt}{3ex} & $2$ & $.04$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.89$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.44$ & $\pm\,0.06$\rule{0pt}{3ex} & $2970$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.13$ & $\pm\,0.02$\rule{0pt}{3ex} & $140$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $55$ & $.8$ & $\pm\,0.6$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.12$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_61_2_2__5.8523785601997256_0.0145656190790761}{WISEA J222116.01$+$005004.0} & $18$ & $.37$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3870$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.10$\rule{0pt}{3ex} & $1700$ &  & $\pm\,400$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.3417$ & $\pm\,0.0004$\rule{0pt}{3ex} & $3$ & $.2$ & $2$ & $.14$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_41_2_2__5.8528504242875199_-0.0003339553862668}{WISEA J222122.46$-$000109.0} & $17$ & $.80$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.41$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.31$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.04$\rule{0pt}{3ex} & $460$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.1067$ & $\pm\,0.0003$\rule{0pt}{3ex} & $2$ & $.0$ & $2$ & $.65$ & 9 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_51_2_0__5.8531779876816650_0.0065602238369244}{WISEA J222126.96$+$002233.1} & $16$ & $.45$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.28$ & $\pm\,0.10$\rule{0pt}{3ex} & $1$ & $.62$ & $\pm\,0.09$\rule{0pt}{3ex} & $0$ & $.80$ & $\pm\,0.07$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.06$\rule{0pt}{3ex} & $3070$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $160$ &  & $\pm\,30$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $4$ & $.132$ & $\pm\,0.003$\rule{0pt}{3ex} & $2$ & $.9$ & $1$ & $.73$ & 36 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_31_3_3__5.8546572070041032_-0.0027362970273606}{WISEA J222147.31$-$000924.4} & $17$ & $.26$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $3930$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.10$\rule{0pt}{3ex} & $1100$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $11$ & $.49$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.5$ & $1$ & $.13$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_30_4_1__5.8581182851243527_-0.0049203048183765}{WISEA J222234.93$-$001655.4} & $17$ & $.42$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.30$ & $\pm\,0.08$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.68$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.04$\rule{0pt}{3ex} & $380$ &  & $\pm\,70$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.867$ & $\pm\,0.002$\rule{0pt}{3ex} & $9$ & $.1$ & $9$ & $.10$ & 37 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/9_40_2_2__5.8584081124837706_-0.0004452579232787}{WISEA J222238.89$-$000132.1} & $16$ & $.88$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.20$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.58$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3380$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.07$\rule{0pt}{3ex} & $420$ &  & $\pm\,80$\rule{0pt}{3ex} & $-1$ & $.8$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $16$ & $.88$ & $\pm\,0.10$\rule{0pt}{3ex} & $4$ & $.1$ & $1$ & $.41$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_27_4_1__6.1286394126535120_-0.0226125360501176}{WISEA J232434.84$-$011744.1} & $17$ & $.10$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.17$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.00$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.50$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $3530$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.45$ & $\pm\,0.08$\rule{0pt}{3ex} & $580$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.2955$ & $\pm\,0.0004$\rule{0pt}{3ex} & $3$ & $.0$ & $2$ & $.96$ & 16 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_57_2_3__6.1298054414349155_-0.0068330663247009}{WISEA J232450.86$-$002329.6} & $16$ & $.21$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3200$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $200$ &  & $\pm\,40$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $19$ & $.9$ & $\pm\,0.3$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.39$ & 14 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_57_1_0__6.1327183134374295_-0.0040443184942774}{WISEA J232530.93$-$001354.2} & $17$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.97$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.22$ & $\pm\,0.05$\rule{0pt}{3ex} & $3530$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.46$ & $\pm\,0.08$\rule{0pt}{3ex} & $620$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $0$ & $.7813$ & $\pm\,0.0007$\rule{0pt}{3ex} & $3$ & $.2$ & $2$ & $.42$ & 19 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_77_1_1__6.1336556654681491_0.0089542380760904}{WISEA J232543.82$+$003046.9} & $18$ & $.01$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.25$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.04$\rule{0pt}{3ex} & $450$ &  & $\pm\,90$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.24$ & $\pm\,0.03$\rule{0pt}{3ex} & $3$ & $.0$ & $3$ & $.00$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_76_2_1__6.1370920910434190_0.0085394272008544}{WISEA J232631.07$+$002921.3} & $18$ & $.91$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.16$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.77$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $3810$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.59$ & $\pm\,0.10$\rule{0pt}{3ex} & $2000$ &  & $\pm\,400$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $15$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $5$ & $.8$ & $1$ & $.17$ & 17 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_56_4_1__6.1377021883452691_-0.0031723063595035}{WISEA J232639.47$-$001054.1} & $17$ & $.47$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.07$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.62$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.12$ & $\pm\,0.05$\rule{0pt}{3ex} & $3860$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.66$ & $\pm\,0.10$\rule{0pt}{3ex} & $1000$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $2$ & $.167$ & $\pm\,0.003$\rule{0pt}{3ex} & $4$ & $.9$ & $2$ & $.34$ & 24 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_36_2_1__6.1378047266608968_-0.0196083463350930}{WISEA J232640.87$-$010724.8} & $17$ & $.76$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.21$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.54$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $3460$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.07$\rule{0pt}{3ex} & $700$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.7$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $75$ & $.8$ & $\pm\,1.0$\rule{0pt}{3ex} & $1$ & $.1$ & $1$ & $.04$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_26_3_2__6.1390035106737848_-0.0220961459684205}{SDSS J232657.36$-$011557.7} & $18$ & $.78$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.29$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.72$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $3100$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.03$\rule{0pt}{3ex} & $530$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $9$ & $.38$ & $\pm\,0.10$\rule{0pt}{3ex} & $3$ & $.2$ & $4$ & $.29$ & 28 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_65_4_1__6.1446425857535507_0.0029951538898682}{WISEA J232814.91$+$001017.6} & $17$ & $.65$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.15$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.37$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.27$ & $\pm\,0.05$\rule{0pt}{3ex} & $3390$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.38$ & $\pm\,0.07$\rule{0pt}{3ex} & $540$ &  & $\pm\,100$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $65$ & $.5$ & $\pm\,0.9$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.05$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_75_3_0__6.1466898175070677_0.0130574338798433}{WISEA J232843.05$+$004453.1} & $16$ & $.40$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.04$\rule{0pt}{3ex} & $3270$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $260$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $107$ &  & $\pm\,2$\rule{0pt}{3ex} & $1$ & $.8$ & $1$ & $.01$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_25_1_3__6.1474207462606962_-0.0252668046063863}{WISEA J232853.08$-$012652.7} & $18$ & $.91$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.26$ & $\pm\,0.07$\rule{0pt}{3ex} & $1$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.73$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $3180$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.23$ & $\pm\,0.04$\rule{0pt}{3ex} & $650$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $75$ & $.4$ & $\pm\,1.0$\rule{0pt}{3ex} & $3$ & $.3$ & $1$ & $.03$ & 15 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_75_1_2__6.1484392965935433_0.0078127598481255}{WISEA J232907.11$+$002651.3} & $17$ & $.05$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.52$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.70$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $3210$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.26$ & $\pm\,0.05$\rule{0pt}{3ex} & $300$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.1$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $1$ & $.3239$ & $\pm\,0.0003$\rule{0pt}{3ex} & $1$ & $.5$ & $1$ & $.27$ & 18 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_44_1_3__6.1541056611439879_-0.0137918805076674}{SDSS J233025.02$-$004724.8} & $17$ & $.54$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.00$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.19$ & $\pm\,0.05$\rule{0pt}{3ex} & $3990$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.10$\rule{0pt}{3ex} & $1100$ &  & $\pm\,200$\rule{0pt}{3ex} & $-1$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $0$ & $.8105$ & $\pm\,0.0002$\rule{0pt}{3ex} & $2$ & $.8$ & $2$ & $.92$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_14_3_2__6.1555055499270948_-0.0294790902094871}{WISEA J233044.27$-$014120.5} & $18$ & $.44$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.23$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.51$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.71$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $3200$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.25$ & $\pm\,0.05$\rule{0pt}{3ex} & $550$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.2$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $93$ &  & $\pm\,2$\rule{0pt}{3ex} & $1$ & $.9$ & $1$ & $.02$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_83_2_1__6.1574726641507569_0.0152352865349061}{WISEA J233111.32$+$005222.3} & $16$ & $.55$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.27$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.38$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.65$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $3270$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.29$ & $\pm\,0.05$\rule{0pt}{3ex} & $280$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.0$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $5$ & $.226$ & $\pm\,0.010$\rule{0pt}{3ex} & $2$ & $.1$ & $3$ & $.65$ & 27 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_33_2_2__6.1582823393093848_-0.0208649412424804}{WISEA J233122.46$-$011143.8} & $18$ & $.35$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.35$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.83$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.05$\rule{0pt}{3ex} & $3030$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.16$ & $\pm\,0.03$\rule{0pt}{3ex} & $360$ &  & $\pm\,80$\rule{0pt}{3ex} & $-2$ & $.5$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.5696$ & $\pm\,0.0005$\rule{0pt}{3ex} & $2$ & $.2$ & $1$ & $.34$ & 21 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_53_3_1__6.1606076287758986_-0.0035961871714288}{WISEA J233154.44$-$001221.9} & $17$ & $.51$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.18$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.36$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.63$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.28$ & $\pm\,0.05$\rule{0pt}{3ex} & $3330$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.34$ & $\pm\,0.06$\rule{0pt}{3ex} & $470$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.1877$ & $\pm\,0.0007$\rule{0pt}{3ex} & $2$ & $.1$ & $1$ & $.75$ & 26 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_63_1_0__6.1627078370731292_0.0007224415329603}{WISEA J233223.32$+$000229.1} & $18$ & $.06$ & $\pm\,0.04$\rule{0pt}{3ex} & $1$ & $.31$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.87$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.88$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $2990$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.13$ & $\pm\,0.02$\rule{0pt}{3ex} & $280$ &  & $\pm\,50$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $14$ & $.75$ & $\pm\,0.04$\rule{0pt}{3ex} & $2$ & $.1$ & $2$ & $.12$ & 13 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_42_4_2__6.1646909038507669_-0.0094898926427581}{WISEA J233250.57$-$003237.3} & $19$ & $.03$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.33$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.75$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.79$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.35$ & $\pm\,0.05$\rule{0pt}{3ex} & $3080$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.18$ & $\pm\,0.03$\rule{0pt}{3ex} & $560$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.4$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $1$ & $.7636$ & $\pm\,0.0007$\rule{0pt}{3ex} & $2$ & $.3$ & $2$ & $.60$ & 12 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_51_4_1__6.1712980477062107_-0.0029202592560150}{WISEA J233421.44$-$001002.2} & $17$ & $.25$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.13$ & $\pm\,0.06$\rule{0pt}{3ex} & $1$ & $.32$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.60$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.30$ & $\pm\,0.05$\rule{0pt}{3ex} & $3410$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.40$ & $\pm\,0.07$\rule{0pt}{3ex} & $450$ &  & $\pm\,90$\rule{0pt}{3ex} & $-1$ & $.9$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $63$ & $.5$ & $\pm\,0.8$\rule{0pt}{3ex} & $1$ & $.6$ & $1$ & $.06$ & 11 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_41_2_1__6.1721956725331459_-0.0131554166363055}{WISEA J233433.77$-$004513.6} & $17$ & $.45$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.24$ & $\pm\,0.05$\rule{0pt}{3ex} & $1$ & $.64$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.78$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.39$ & $\pm\,0.05$\rule{0pt}{3ex} & $3120$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.20$ & $\pm\,0.04$\rule{0pt}{3ex} & $290$ &  & $\pm\,60$\rule{0pt}{3ex} & $-2$ & $.3$ & $\pm\,0.2$\rule{0pt}{3ex} &  & $3$ & $.177$ & $\pm\,0.004$\rule{0pt}{3ex} & $3$ & $.7$ & $2$ & $.04$ & 30 \\
\href{http://ps1-mds-variability-classifier.appspot.com/star/10_41_2_0__6.1726753155778376_-0.0113098415681158}{WISEA J233440.36$-$003853.0} & $19$ & $.85$ & $\pm\,0.03$\rule{0pt}{3ex} & $1$ & $.19$ & $\pm\,0.09$\rule{0pt}{3ex} & $1$ & $.87$ & $\pm\,0.06$\rule{0pt}{3ex} & $0$ & $.89$ & $\pm\,0.05$\rule{0pt}{3ex} & $0$ & $.41$ & $\pm\,0.05$\rule{0pt}{3ex} & $3020$ &  & $\pm\,80$\rule{0pt}{3ex} & $0$ & $.17$ & $\pm\,0.03$\rule{0pt}{3ex} & $610$ &  & $\pm\,100$\rule{0pt}{3ex} & $-2$ & $.6$ & $\pm\,0.2$\rule{0pt}{3ex} & ? & $5$ & $.26$ & $\pm\,0.02$\rule{0pt}{3ex} & $7$ & $.6$ & $2$ & $.70$ & 30
\enddata
\end{deluxetable}
% end TableBuilder table

